Enabling Non-Linear Quantum Operations through Variational Quantum Splines

The postulates of quantum mechanics impose only unitary transformations on quantum states, which is a severe limitation for quantum machine learning algorithms. Quantum Splines (QSplines) have recently been proposed to approximate quantum activation functions to introduce non-linearity in quantum algorithms. However, QSplines make use of the HHL as a subroutine and require a fault-tolerant quantum computer to be correctly implemented. This work proposes the Generalised Hybrid Quantum Splines (GHQSplines), a novel method for approximating non-linear quantum activation functions using hybrid quantum-classical computation. The GHQSplines overcome the highly demanding requirements of the original QSplines in terms of quantum hardware and can be implemented using near-term quantum computers. Furthermore, the proposed method relies on a flexible problem representation for non-linear approximation and it is suitable to be embedded in existing quantum neural network architectures. In addition, we provide a practical implementation of the GHQSplines using Pennylane and show that our model outperforms the original QSplines in terms of quality of fitting.

==> discussion.tex <==
The GHQSplines algorithm uses a problem formulation that allows obtaining an end-to-end quantum algorithm representing the spline coefficients with a single linear system of equations. In this case, results are more stable, the shape of the curve is well-approximated, and the non-linearity is well-captured. However, while a higher number of knots improves the fitting by building smaller intervals, it also increases the normalization penalty on $\ket{Y}$ and $\ket{\beta}$. To tackle this problem, one can consider adopting amplitude amplification \cite{Brassard2000} to stretch the shape of the curve and increase the amplitudes to correct the normalization effects.\\
Furthermore, to use of GHQSplines as a method for quantum activation functions requires the ability to calculate the target variable $\hat{y_j}$ from a generic input $x_j$. In this regard, we have to devise a mapping circuit $M$ that creates a vector representing the basis expansion of $x_j$. 
Then, in order to obtain $\hat{y}_j$ we have to apply the dot-product between the basis expansion of $x_j$ and the $\beta$ coefficients, both encoded as a quantum state.
The only difference between this approach and the one described for the GHQSplines is that here the Ansatz ($V^\dag$) is transposed and applied in reverse order with respect to the encoding of the basis expansion of $x_j$. This procedure allows the proposed GHQSplines method to produce a non-linear function $f$ for a given input $x_j$ which approximates the target variable $y$. 

